Text-Adaptive Multiple Visual Prototype Matching for Video-Text Retrieval

Cross-modal retrieval between videos and texts has gained increasing research interest due to the rapid emergence of videos on the web. Generally, a video contains rich instance and event information and the query text only describes a part of the information. Thus, a video can correspond to multiple different text descriptions and queries. We call this phenomenon the ``Video-Text Correspondence Ambiguity'' problem. Current techniques mostly concentrate on mining local or multi-level alignment between contents of a video and text (\textit{e.g.}, object to entity and action to verb). It is difficult for these methods to alleviate the video-text correspondence ambiguity by describing a video using only one single feature, which is required to be matched with multiple different text features at the same time. To address this problem, we propose a Text-Adaptive Multiple Visual Prototype Matching model, which automatically captures multiple prototypes to describe a video by adaptive aggregation of video token features. Given a query text, the similarity is determined by the most similar prototype to find correspondence in the video, which is termed text-adaptive matching. To learn diverse prototypes for representing the rich information in videos, we propose a variance loss to encourage different prototypes to attend to different contents of the video. Our method outperforms state-of-the-art methods on four public video retrieval datasets.

==> didemo.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{|c|cccc|}
\hline
\multirow{2}{*}{Method}      & \multicolumn{4}{c|}{Text-to-Video}                                                                           \\ \cline{2-5} 
                             & \multicolumn{1}{c|}{R@1}  & \multicolumn{1}{c|}{R@5}  & \multicolumn{1}{c|}{R@10} & MedR                     \\ \hline
S2VT  \cite{S2VT}                      & \multicolumn{1}{c|}{11.9} & \multicolumn{1}{c|}{33.6} & \multicolumn{1}{c|}{-}    & 13.0                     \\
FSE  \cite{FSE}                     & \multicolumn{1}{c|}{13.9} & \multicolumn{1}{c|}{36.0} & \multicolumn{1}{c|}{-}    & 11.0                     \\
TT-CE+   \cite{TT-CE+}                   & \multicolumn{1}{c|}{21.6} & \multicolumn{1}{c|}{48.6} & \multicolumn{1}{c|}{62.9} & 6.0                      \\ \hline
CE    \citep{CE}                        & \multicolumn{1}{c|}{16.1} & \multicolumn{1}{c|}{41.1} & \multicolumn{1}{c|}{-}    & 8.3                      \\
\hline
ClipBERT   \citep{ClipBERT}                   & \multicolumn{1}{c|}{20.4} & \multicolumn{1}{c|}{48.0} & \multicolumn{1}{c|}{60.8} & 6.0                      \\
\multicolumn{1}{|c|}{Frozen \cite{Frozen} } & \multicolumn{1}{c|}{31.0} & \multicolumn{1}{c|}{59.8} & \multicolumn{1}{c|}{72.4} & \multicolumn{1}{c|}{3.0} \\
\hline 
Ours                         & \multicolumn{1}{c|}{36.5} & \multicolumn{1}{c|}{67.4} & \multicolumn{1}{c|}{81.3} & 16.0                     \\ \hline
\end{tabular}
\end{table}


% \begin{table}[]
% \begin{tabular}{|c|cccc|}
% \caption{Retrieval performance on the MSVD dataset}
% \hline
% \multirow{2}{*}{Method}      & \multicolumn{4}{c|}{Text-to-Video}                                                                           \\ \cline{2-5} 
%                              & \multicolumn{1}{c|}{R@1}  & \multicolumn{1}{c|}{R@5}  & \multicolumn{1}{c|}{R@10} & MedR                     \\ \hline
% VSE  \cite{VSE}                       & \multicolumn{1}{c|}{12.3} & \multicolumn{1}{c|}{30.1} & \multicolumn{1}{c|}{42.3} & 14.0                     \\
% VSE++  \cite{VSE++}                      & \multicolumn{1}{c|}{15.4} & \multicolumn{1}{c|}{39.6} & \multicolumn{1}{c|}{53.0} & 9.0                      \\
% TT-CE+  \cite{TT-CE+}   & \multicolumn{1}{c|}{25.4} & \multicolumn{1}{c|}{56.9} & \multicolumn{1}{c|}{71.3} & \multicolumn{1}{c|}{4.0} \\
% SUPPORT\_SET   \citep{SupportSet}                  & \multicolumn{1}{c|}{28.4} & \multicolumn{1}{c|}{60.0} & \multicolumn{1}{c|}{72.9} & 4.0                      \\
% \hline
% MC \cite{MC}                 & \multicolumn{1}{c|}{20.3} & \multicolumn{1}{c|}{47.8} & \multicolumn{1}{c|}{61.1} & 6.0                      \\
% CE  \cite{CE}                        & \multicolumn{1}{c|}{19.8} & \multicolumn{1}{c|}{49.0} & \multicolumn{1}{c|}{63.8} & 6.0                      \\
% \hline
% Frozen  \cite{Frozen}                     & \multicolumn{1}{c|}{33.7} & \multicolumn{1}{c|}{64.7} & \multicolumn{1}{c|}{76.3} & 3.0                      \\ \hline
% Ours                         & \multicolumn{1}{c|}{36.5} & \multicolumn{1}{c|}{67.4} & \multicolumn{1}{c|}{81.3} & 3.0                      \\ \hline
% \end{tabular}
% \end{table}
